Minimum Strict Consistent Subset in Paths, Spiders, Combs and Trees

Let G be a simple connected graph with vertex set V(G) and edge set E(G. Each vertex of V(G) is colored by a color from the set of colors {c_1, c_2,\dots, c_{\alpha}}. We take a subset S of V(G), such that for every vertex v in V(G)\S, at least one vertex of the same color is present in its set of nearest neighbors in S. We refer to such an S as a consistent subset (CS). The Minimum Consistent Subset (MCS) problem is the computation of a consistent subset of the minimum cardinality. It is established that MCS is NP-complete for general graphs, including planar graphs. The strict consistent subset is a variant of consistent subset problems. We take a subset S^{\prime} of V(G), such that for every vertex v in V(G)\S^{\prime}, all the vertices in its set of nearest neighbors in S^{\prime} have the same color as that of v. We refer to such an S^{\prime} as a strict consistent subset (SCS). The Minimum Strict Consistent Subset (MSCS) problem is the computation of a strict consistent subset of the minimum cardinality. We demonstrate that MSCS is NP-hard for general graphs using a reduction from dominating set problems. We construct a 2-approximation algorithm and a polynomial-time algorithm in trees. Lastly, we conclude the faster polynomial-time algorithms in paths, spiders, and combs.

==> MCSTreeHard.tex <==
\section{\np-hardness of MCS for Trees} \label{hardnesstree}
In this section, we prove that \csp is \nph ~even when the input graph is a tree. We present a reduction from MAX-2SAT problem to \csp. Let $\theta$ be a given MAX-$2$SAT formula with $n$ variables $\{x_1, \ldots, x_n\}$ and $m$ clauses $\{c_1, \ldots, c_m\}$, $n,m \geq 50$. We construct an instance $(T_{\theta}, C_{\theta})$ of the MCS problem from $\theta$ as follows.


%reduce an arbitrary given instance $\theta$ of the MAX-2SAT problem to an instance $(T_{\theta}, C_{\theta})$ of the MCS problem where $T_{\theta}$ is a tree. 

%Here,  $k$ clauses of $\theta$ can be satisfied if and only if the reduced tree $T$ has a consistent subset of a certain size (depending on $k$) that we describe later on.
%Throughout this section, by distance between two vertices in $T$, we refer to the hop-distance between them. The distance between a vertex $v$ and a path is the minimum distance between $v$ and any vertex of that path. The distance between two paths $P_1$ and $P_2$ in $T$ is the minimum distance of a pair vertices $v_1\in P_1$ and $v_2\in P_2$.


\begin{figure}[t]
\centering
\includegraphics[width=0.8\textwidth]{treehardness.pdf}
\caption{An example of construction of $(T_{\theta}, C_{\theta})$ where $\theta=(x_1\lor x_2)\land (x_1\lor \overline{x_3})\land (\overline{x_2}\lor \overline{x_3}))$. For the assignment $x_1=x_2=x_3=\false$, we have shown the corresponding \cs with a red box around the vertices. For the mentioned assignment,  $(x_1\lor x_2)$ is not satisfied whereas the rest of the clauses are satisfied} \label{fig:red}
\end{figure}


%\subsection{Construction of $(T_{\theta}, C_{\theta})$}


\vspace{-0.2in}
\begin{tcolorbox}[breakable,bicolor,
  colback=cyan!5,colframe=cyan!5,title=Interval Graph Construction.,boxrule=0pt,frame hidden]


% \begin{mdframed}[backgroundcolor=cyan!5,topline=false,bottomline=false,leftline=false,rightline=false]
\noindent \underline{\textbf{\large Construction of $(T_{\theta}, C_{\theta})$.}}
%\noindent \paragraph{Reduction.}
%\subsection{Reduction}
\smallskip

\noindent The constructed tree $T_{\theta}$ is composed of variable and clause gadgets. 
\smallskip

\noindent {\bf Variable Gadget.}

\noindent A variable gadget $X_i$ for the variable $x_i \in \theta$ has two components, each component has a literal path, and $M$ pairs of stabilizer vertices, as described below (see Figure \ref{fig:red}), where $M$ is very large.


\smallskip

\noindent {\bf Literal paths:} The two literal paths of the variable gadget $X_i$ are $P^\ell_i=\langle x_i^1, x_i^2,x_i^3,x_i^4\rangle$ and $\overline{P}^\ell_i = \langle \overline{x}_i^1,\overline{x}_i^2,\overline{x}_i^3, \overline{x}_i^4\rangle$, each consisting of four vertices; these are referred to as \emph{positive literal path}, and \emph{negative literal path} respectively. Here, by a path of $k$ ($> 2$) vertices, we mean a connected graph with $k-2$ nodes having degree 2 and the remaining two nodes having degree 1. All the vertices on the path $P_i^\ell$ are of color $c^\ell_i$ and all the vertices on the path $\overline{P}_i^\ell$ are of color $\overline{c}^\ell_i$.
 
 %In each path, all its nodes have the same color, and these two paths have different colors. The path $x_i$ corresponds to $x_i=1$, and path $\overline{x_i}$ corresponds to $\overline{x_i}=1$ (i.e. $x_i=0$).
\smallskip

\noindent {\bf Stabilizer vertices:} $M$ pairs of vertices $\{s_{i}^1, \overline{s}_i^1\}, \ldots, \{s_{i}^M, \overline{s}_i^M\}$ (we will define the exact value of $M$ later), where the color of each pair of vertices $\{s_{i}^j, \overline{s}_i^j\}$ is $c^s(i,j)$. We denote the set of vertices $S_i=\{ s_{i}^1,  \ldots, s_{i}^M\}$ as  \emph{positive stabilizer vertices} and the set of vertices $\overline{S}_i=\{\overline{s}_i^1, \ldots,  \overline{s}_i^M\}$ as \emph{negative stabilizer vertices}. Each vertex in $S_i$ is connected to $x_i^1$ and each vertex in $\overline{S}_i$ is connected to $\overline{x}_i^1$.

The intuition behind this set of stabilizer vertices is that by setting a large value of $M$ we ensure that either $\{s_{i}^1,  \ldots, s_{i}^M\}$ or $\{\overline{s}_i^1, \ldots,  \overline{s}_i^M\}$ is present in any "small" sized solution. 

%The vertices of the form $s_{i,j}^1$ are called the \emph{left stabilizers} while those of the form $s_{i,j}^2$ are called the right stabilizers. Each pair of stabilizer vertices have the same color, and these $M$ pairs of stabilizer vertices have distinct colour, which are also different from that of the vertices in variable paths and literal paths. The left (resp. right) stabilizer vertices are connected with the first vertex of left (resp. right) literal paths. 
%\end{description}

\smallskip

\noindent {\bf Clause Gadget.}

\noindent For each clause $c_i=(y_i\lor z_i)$, where $y_i$ and $z_i$ are two (positive/negative) literals, we define the clause gadget $C_i$ as follows. It consists of three paths, namely \emph{left occurrence path} $P_i^Y=\langle y_i^1,\cdots y_i^7\rangle$, \emph{right occurrence path} $P_i^Z=\langle z_i^1,\cdots z_i^7\rangle$, and {\em clause path} $P_i^W=\langle w_i^1,\cdots w_i^7\rangle$ (see Figure \ref{fig:red}).
All the vertices in $P_i^Y$ (resp. $P_i^Z$) have the same color as that of the corresponding literal path in their respective variable gadgets, i.e. for any literal, say $y_i$, in $C_i$ if $y_i=x_i$ (resp. $\overline{x_i}$) then we set the color of the vertices of $P_i^Y$ as $c_i^x$ (resp. $\overline{c}_i^x$). The color of the vertices on the path $P_i^Z$ is set in the same manner. We color the vertices in $P_i^W$ by $c^w_i$, which is different from that of the vertices in $P_i^Y$ and $P_i^Z$.
We create the clause gadget $C_i$ by connecting $y_i^1$ with $w_i^2$ and $z_i^1$ with $w_i^6$ by an edge (see Figure \ref{fig:red}).

\smallskip

\noindent {\bf Central Vertex Gadget.}

\noindent We also have a central path $P^v=\langle v_1,v_2, v_3\rangle$. The color of all the vertices in $P^v$ are same, say $c^v$, which is different from the color of all other vertices in the construction. For each variable gadget $X_i$,  $x_i^1$ and $\overline{x}_i^1$ are connected with the vertex $v_1$ (see Figure \ref{fig:red}). For each clause $C_i$, $w_i^4$ is connected with $v_1$. Color of the vertices of $P^v$  is $c^v$.


%\end{mdframed}

\end{tcolorbox}

% Another part of this reduction is a 
% vertex $v$, named central vertex, and it is attached with a path of length (including $v$), called the central path. The vertices of central path is different from all the  vertices in variable gadgets and clause gadgets. Now, we explain how the variable and clause gadgets are connected to form the tree $T$.

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.9\textwidth]{mcspic5a.pdf}
% \caption{A part of the reduction tree demonstrating one variable gadget $x_i$, and one clause gadget $c_\alpha$. For a truth assignment of $x_i=1$, the vertices included in the minimum consistent subset $S$ are enclosed with a square box. } \label{fig:red}
% \end{figure}

% \begin{enumerate}
% \item The two components of each variable gadget are individually connected with the central vertex $v$. 
% \item As mentioned earlier, the middle vertex of each clause gadget is connected with the central vertex $v$. 
% \end{enumerate}

Our objective is to show that there exists an \mcs of size at most $N(k)=n(M+2)+2k+3(m-k)+1$ in the tree $T_\theta$ if at least $k$ clauses of $\theta$ are satisfied; otherwise, it is strictly greater than $N(k)$. 
We now prove a set of auxiliary claims about a minimum consistent subset for $(T_{\theta}, C_{\theta})$. 

{Lemma \ref{lemma:exactlyone}, stated below, says that by judiciously choosing the vertices in a variable gadget, the vertices of the tree corresponding to that variable gadget can be consistently covered by choosing its only one set of stabilizer vertices.}

\begin{lemma} \label{lemma:exactlyone}
For any consistent subset $V_C$ of size at most $N(k)=n(M+2)+2k+3(m-k)+1$ in the tree $T_\theta$, the following are true.
\begin{itemize}
    \item For any variable $x_i$, exactly one of the following is true.
        \begin{itemize}
            \item $S_i\subset V_C$, $\overline{S}_i\cap V_C=\emptyset$, and $x_i^2,\overline{x}_i^4\in V_C$. 
            \item $\overline{S}_i\subset V_C$, ${S}_i\cap V_C=\emptyset$, and $\overline{x}_i^2,x_i^4\in V_C$, and  
        \end{itemize}
    \item $v_3\in V_C$.
\end{itemize}
\end{lemma}
    \begin{proof}
     For a variable $x_i$, let $S_i\cap V_C \neq \emptyset$. Let $s_i^j\in S_i\cap V_C$. But then every vertex $v \in S_i\setminus \{s_i^j\}$ must have a vertex within distance 2 of its own color, since $dist(s_i^j,v)=2$. Hence $S_i\subset V_C$. One can similarly prove that $\overline{S}_i\cap V_C \neq \emptyset
      \implies \overline{S}_i\subseteq V_C$.
     Also, every variable gadget contains $M$ uniquely colored vertices and hence has at least $M$ vertices in $V_C$. So, if $M>>n$, we have that $N(k)<(n+1)M$, and there exists no variable gadget that contains vertices from both $S_i$ and $\overline{S}_i$. In other words exactly one of the following holds for every variable gadget corresponding to a variable $x_i$: 
     \begin{itemize}
     \item  $S_i\subset V_C$, $\overline{S}_i\cap V_C=\emptyset$
     \item $\overline{S}_i\subset V_C$, ${S}_i\cap V_C=\emptyset$,
     \end{itemize}

     Below, we look into one of these cases, and a similar argument may be made for the other case as well.

     \noindent\textbf{\underline{Case 1: $S_i\subset V_C$, $\overline{S}_i\cap V_C=\emptyset$}}

     Notice that there must be a vertex in the literal path \{$x_i^1,x_i^2,x_i^3,x_i^4$\} from \{$x_i^1,x_i^2$\} of the variable gadget $X_i$ since $dist(S_i,x_i^1)=1$ and the distance to any other vertex of the same color (other than these two vertices) is more than 1. But $x_i^1 \notin V_C$, as $\overline{S}_i\cap V_C=\emptyset$ and $dist(x_i^1,\overline{S}_i)< dist(S_i,\overline{S}_i)$. Hence $x_i^2 \in V_C$.

     Similarly there must be a vertex in the literal path $\{\overline{x}_i^1,\overline{x}_i^2,\overline{x}_i^3,\overline{x}_i^4\}$ of the variable gadget $X_i$ since $dist(S_i,\overline{x}_i^1)=3$ and the distance to any other vertex of the same color (other than $\{\overline{x}_i^2,\overline{x}_i^3,\overline{x}_i^4\}$) is more than 3. And the distance of 4 between $S_i$ and $\overline{S_i}$ eliminates the possibility of belonging any of the vertices $\overline{x}_i^1,\overline{x}_i^2,\overline{x}_i^3$ in $V_C$. Thus, $\overline{x}_i^4\in V_C$ 

     \noindent\textbf{\underline{Case 2: $\overline{S}_i\subset V_C$, ${S}_i\cap V_C=\emptyset$}} 
     
     Case 2 may be argued in a manner similar to Case 1.


     
     
   Moreover, there needs to be a vertex within the set $\{v_1, v_2, v_3\}$. However, the distance of 4 between $S_i$ and $\overline{S_i}$ rules out the possibility of either $v_1$ or $v_2$ being in $V_C$. Consequently, $v_3 \in V_C$.           \end{proof}
   
%Thus, Lemma \ref{lemma:exactlyone} says that there exists a set of $M=(n(M+2)+1)$ vertices which defines a consistent subset of a subtree of $T_\theta$ consisting of the central vertex gadget and the variable gadgets of all the variables in $\theta$. 
To satisfy the inequality in the above lemma, we now set the value of $M$ as $n^3$.
In the next lemma, we present a bound on the vertices from each clause gadget that are contained in a consistent subset of size at most $N(k)$.
For any clause $C_i$, denote the corresponding clause gadget by $T_i^C=G[\{w_i^a,y_i^a,z_i^a|1\leq a\leq 7\}]$.
    \begin{lemma}
        In any consistent subset $V_C$ of the tree $T_\theta$, for each clause $C_i$, $2\leq |V(T_i^C)\cap V_C|$.\label{lemma:clause2or3}
    \end{lemma}
    \begin{proof}
There needs to be a vertex among the vertices $\{w_i^a \mid 1 \leq a \leq 7\}$ since they are distinctly colored from all other vertices. If this vertex belongs to $\{w_i^a \mid 1 \leq a \leq 4\}$, then there must also be a vertex in $\{y_i^a \mid 1 \leq a \leq 7\}$ since the nearest vertex of the same color (any $y_i^a$) is farther away than the vertex with the color of any $w_i^a$. Similarly, if this vertex belongs to $\{w_i^a \mid 4 \leq a \leq 7\}$, then there must be a vertex in $\{z_i^a \mid 1 \leq a \leq 7\}$. Therefore, $2 \leq |V(T_i^C)\cap V_C|$.
    \end{proof}


 %Now, our objective is to choose the vertices in the clause gadgets such that we can get a \mcs maintaining the contribution of $M$ number of vertices from the central path gadget and all the variable gadgets. 



% \begin{lemma}
% With a truth assignment of the variables of $T_\theta$, if the vertices in the variable gadgets and central path gadget are done as stated in Lemma \ref{1stabilizer}, then 

% \begin{itemize}
% \item[(i)] if a clause $c_i=y_i+z_i$ is satisfied, then in the corresponding clause gadget $C_i=G[\{w_i^a,y_i^a,z_i^a|1\leq a\leq 7\}]$, exactly 2 vertices are enough to choose in \mcs to consistently cover all the vertices in $C_i$, and \item[(ii)] if a clause $c_i=y_i+z_i$ is not satisfied, then 3 vertices are necessary in the corresponding clause gadget to make all the vertices in $C_i$ consistently covered.
% \end{itemize}
% \end{lemma}
% \begin{proof}
% Note that, we need to choose at least one vertex of the clause path $P_i^W$ in the clause gadget $C_i$ since no vertex of that color appears in the constructed tree $T_\theta$ irrespective of whether 0 or 1 or 2 literals are satisfied by the truth assignments of the variables of $\theta$.

% {\bf Part (i)} A satisfied clause $c_i=y_i+z_i$ has either one or two literals that are satisfied by the truth assignment of the variables in $\theta$.
% \begin{itemize} 
% \item If only one literal, say $y_i$ (uncomplemented or complemented $x_j$), is satisfied, then we include the first vertex $z_i^1$ of the occurrence path of $z_i$ and the vertex $w_i^7$, i.e., the end-vertex of the clause path in the side where $P_i^Z$ is connected. Needless to say,  (i) all the vertices of the occurrence path of $P_i^Z$ are satisfied for choosing $z_i^1$; (ii) $w_i^4$ is satisfied since $d(w_i^4,w_i^7) = d(w_i^4,z_i^1)=d(w_i^4,x_j^2)=3$, where $x_j^2$ is the chosen vertex in literal path $P_j^\ell$ as $x_j=1$ is set, $w_i^7$ is the chosen vertex in the clause path $P_i^W$, and $z_i^1$ is the chosen vertex in the occurrence path $P_i^Z$.  This implies, all the vertices on the clause path $P_i^W$ and all the vertices on the occurrence path $P_i^Y$ are satisfied.   

% \item If both the literals $l_i$ and $l_j$ are satisfied by the truth assignment of the variables in $\theta$, then, as mentioned earlier, we need to choose at least one vertex on the clause path $P_i^W$ to make its vertices consistent. Here also, we choose the same two vertices as was done in the earlier case. 
% \end{itemize}
%  Thus, the result in Part (i) follows. 
 
% {\bf Part (ii)} If $c_i=y_i+z_i$ is unsatisfied in the truth assignment of the variables in $\theta$. Let $y_i$ and $z_i$ correspond to the variables $x_j$ and $x_{j'}$ respectively (in uncomplemented or complemented form). Thus, the distance of $w_i^4 \in P_i^W$ (on the clause path) is at distance 
% 5 from the chosen vertices in the variable gadgets $Y_i$ and $Z_i$, that have the same color as that of the color of the path $P_i^Y$ and $P_i^Z$ respectively. To make it consistent, we choose any one vertex (say $w_i^\alpha$, $\alpha\neq 4$) of the clause path; this forces us to choose one appropriate vertex from each of the occurrence paths $P_i^Y$ and $P_i^Z$, so that all the vertices of both the occurrence paths and the clause path are consistently covered.  Thus, the result of Part (ii) follows. 
% \end{proof}

\begin{theorem}
    There exists a truth assignment of the variables in $\theta$ which satisfies at least $k$ clauses if and only if there exists a consistent subset of size at most $N(k)$ for $(T_{\theta},C_{\theta})$.
\end{theorem}

\begin{proof}
$(\Rightarrow)$ For the forward direction, let there exist an assignment $A$ to the variables of $\theta$ that satisfies $k$ clauses. Consider the following set of vertices $V_A$. For each variable $x_i$ if $x_i$ is $\true$, include all the vertices of $S_i$ in $V_A$. Also include $x_i^2$ and $\overline{x}_i^4$ in $V_A$. If $x_i=\false$ then include all the vertices of $\overline{S}_i$ in $V_A$. Also include $x_i^4$ and $\overline{x}_i^2$ in $V_A$.

For every satisfied clause $C_i=(y_i\lor z_i)$ with respect to $A$ we include the following vertices in $V_A$. Without loss of generality assume that $y_i=\true$. We include $w_i^7$ and $z_i^1$ in $V_A$.
For every unsatisfied clause $C_i=(y_i\lor z_i)$, we include  $w_i^1$, $y_i^1$ and  $z_i^7$ in $V_A$. We also include $v_3$ in $V_A$.

Observe that the cardinality of $V_A$ is $N(k)=n(M+2)+2k+3(m-k)+1$. Next, we prove that $V_A$ is a consistent subset for $T_{\theta}$. Observe that for any pair of vertices $(s_i^j,\overline{s}_i^j)$, exactly one of them is in $V_A$. Without loss of generality assume that $s_i^j\in V_A$. Observe that $d(s_i^j,\overline{s}_i^j)=d(\overline{s}_i^j,V_A)=4$. If $x_i=\true$ then $d(x_i^j,x_i^2)\leq d(x_i^j,V_A)$ and $d(\overline{x}_i^j,\overline{x}_i^4)\leq d(\overline{x}_i^j,V_A)$. The case when $x_i=\false$ is symmetric.

For any clause gadget either $w_i^1$ or $w_i^7$ is in $V_A$. Without loss of generality assume that $w_i^1\in V_A$. Observe that for every vertex $w_i^j$, $d(w_i^j,w_i^1)=d(w_i^j.V_A)$. Let $C_i=(y_i\lor z_i)$ be a satisfied clause and without loss of generality assume that $y_i=x_j=\true$. Observe that $d(y_i^1,x_j^2)=6$, and $d(y_i^3,V_A)=6$, and $d(y_i^a,x_j^2)=d(y_i^a,V_A)$.
For any unsatisfied clause $C_i=(y_i\lor z_i)$ observe that $d(y_i^a,x_j^2)=d(y_i^a,V_A)$. Also for any $v_j$ where $1\leq j\leq 3$ $d(v_j,v_3)=d(v_j,V_A)$. Therefore $V_A$ is a consistent subset for $T_{\theta}$. 
    
    \smallskip
\noindent $ (\Leftarrow) $
In the backward direction,let there be a consistent subset $V_C$ of size at most $N(k)$ for $(T_{\theta},C_{\theta})$. We know from Lemma~\ref{lemma:exactlyone} that either $S_i\subset V_C$ or $\overline{S}_i\subset V_C$. From Lemma~\ref{lemma:exactlyone} any such solution has at least $n(M+2)+1$ facilities outside the clause gadgets leaving at most $2k+3(m-k)$ that may be chosen from the clause gadgets.

Each clause gadget comprises of vertices of three distinct colors: one color exclusive to the clause itself and two colors dedicated to literals. An essential insight is that if there are no facilities of colors specific to the literals from a clause in the variable gadgets, then such a clause gadget must contain at least three facilities. This assertion is valid because the distance between two sets of vertices of the same color (corresponding to the same literal in two clauses) across any two clauses is at least 8, while facilities of clause-specific colors are at a distance of at most 6.

This fact coupled with Lemma~\ref{lemma:clause2or3} implies that there are at least k clauses for whom   colors specific to at least one of their literals have facilities of same color in $V_C$ from the variable gadgets. Making the same literals true and setting other variables aribitrarily gives us an assignment that satisfies at least $k$ clauses.  
\end{proof}







% $ For the backward direction, let there be a consistent subset $V_C$ of size at most $N(k)$ for $(T_{\theta},C_{\theta})$. 
% We known from Lemma~\ref{lemma:exactlyone} that either $S_i\subset V_C$ or $\overline{S}_i\subset V_C$.
% Consider the following assignment $A$ corresponds to $V_C$. For any variable $x_i$ if $S_i\subset V_C$ we set $x_i=\true$, otherwise we set $x_i=\false$. 
    
% Observe that any clause $C_i$, $V_C$ either contains $w_i^1$ or $w_i^7$. Note that $|V_C|=n(M+2)+2k+3(n-k)+1$ and $V_C$ contains $M$ vertices from each variable gadget and $v_3\in V_C$ (follows from Lemma~\ref{lemma:exactlyone} and Lemma~\ref{lemma:clause2or3}). From pigeonhole principle there exist $k$ clause $C_j=(y_j\lor z_j)$ such that either $V(P_j^Y)\cap V_C=\emptyset$ or  $V(P_j^Z)\cap V_C=\emptyset$. Without loss of generality assume that $C_1\cdots C_k$ be such clauses and for all $1\leq j\leq k$, $V(P_j^Y)\cap V_C=\emptyset$. Consider any clause $C_j$ where $1\leq j\leq k$. Without loss of generality assume $y_j=x_i$. Observe that $d(y_j^1,w_j^7)=6$. Thus $x_i^2\in V_C$ and hence $S_i\in V_C$. Therefore $x_i=\true$ in $A$. Hence $C_j$ is satisfied for the assignment $A$. Thus the claim holds.






==> MCStrees.tex <==
\section{\mcs for Trees: A Parameterized Algorithm} \label{fpt}

In this section, we consider the optimization version of the MCS problem for the trees. 
%We will use bottom-up dynamic programming to find the optimal consistent subset. 
\defparproblem{\textsc{Minimum Consistent Subset for Trees} }
{A rooted tree $T$, whose vertices $V$ are coloured with a set $C$ of $c$ colours.}
{$c$}
{Find the minimum possible size of a consistent subset (\mcs) for $T$?}

We consider $T$ as a rooted tree by taking an arbitrary vertex $r$ as its root. We use (i) $V(T')$ to denote the vertices of a subtree $T'$ of $T$, (ii) $C(U) \subseteq C$ to denote the subset of colors assigned to subset of vertices $U  \subseteq V$, and $C(u)$ to denote the color attached to the vertex $u \in V(T)$.
For any vertex $v$, let $\eta_v$ denote the number of children of $v$  and we denote the children of $v$ by $v_1,v_2,\cdots, v_{\eta_v}$. We denote the subtree rooted at a vertex $v$ by $T(v)$. For any vertex $v$ and any integer $i<\eta_v$, we use $T_{i+}(v)$ to denote the union of subtrees rooted at $v_{i+1}$ to $v_{\eta_v}$, and $T_i(v)$ to denote the subtree rooted at $v$ and containing first $i$ many children of $v$. Thus, $T_{i+}(v)=\cup_{i+1\leq j\leq \eta_v}T(v_j)$, which is a forest, and $T_i(v)=T(v)\setminus T_{i+}(v)$. In Figure \ref{fig:dp}, the light yellow part is $T_i(v)$, and the light sky-colored part is $T_{i+}(v)$. 

\begin{figure}[ht]
                \centering
                \includegraphics[scale=1.2]{mcst}
                \caption{\textit{Illustration of the bottom-up dynamic programming routine: The tree inside the triangle is $T_i(v)$, and the forest inside the rectangle is $T_{i+}(v)$}}
                \label{fig:dp}
\end{figure}

For any positive integer $d$ and for any vertex $v\in V(T)$, a set of vertices $U\subset V(T)$ is called $d$-equidistant from $v$ if $d(u_i,v)=d$ for all $u_i\in U$. Any subset of vertices $U$ spans a set of colors $C' \subseteq C$ if $C(U)=C'$. 
%and $C^{-1}(C')=U$\red{every vertex $u \in U$ has a color $c \in C'$, and --- IS IT REQUIRED?} for each color $c\in C'$ there exists a vertex in $U$ which is assigned the color $c$; formally, $C(U)=C'$. 
For any vertex $v\in V(T)$, we use $\Esib(v,d,C')$ (resp. $\Eout(v,d,C')$) to denote the set of subsets of vertices in $T_{i+}(v)$ (resp. $T\setminus T(v)$), which are $d$-equidistant from $v$ and span the colors in $C'$. 
Next, we define a ({\em partial}) {\em consistent subset} for a subtree $T_i(v)$.

%It is intuitively defined as a set of vertices $W\subseteq V(T_i(v))$ defined with respect to six parameters, $d^{\inn},d^{\out},d^{\sib},C^{\inn},C^{\out},C^{\sib}$. Here $d^{\inn}\in\mathbb{Z}_0^+$, $d^{\out},d^{\sib}\in\mathbb{Z}^+$ and $C^{\inn},C^{\out}$ and $C^{\sib}$ are subset of colors in $C$.
%We always define a (partial) consistent subset $W\subseteq V(T_i(v))$ with respect to $d^{\inn},d^{\out},d^{\sib},C^{\inn},C^{\out},C^{\sib}$ with the assumption that there exist a subset of vertices $X\in \Esib(v,d^{\sib},C^{\sib})$ and a subset of vertices $Y\in \Eout(v,d^{\out},C^{\out})$, such that the following conditions are satisfied. The nearest neighbour from $v$ to $W$ is at distance $d^{\inn}$ and for every vertex $u\in T(v)$, $C(u)\in C(\NN(u,W\cup X\cup Y))$. 
%Next, we formally define a (partial) consistent subset for $T_i(v)$. For ease of notation, we will denote a (partial) consistent subset for $T_i(v)$ as a consistent subset for $T_i(v)$.


%A consistent subset $W \subset S_T$ of the subtree of $T_i(v)$ rooted at $v$ with the first $i$ children of $v$, depends on the presence of the vertices of $S_T\cap T_{i+}(v)$ and $S_T\cap (T\setminus T(v))$. This motivates us to define the following:

\begin{definition}
Let $d^{\inn}\in\mathbb{Z}_0^+$, $d^{\out},d^{\sib}\in\mathbb{Z}^+$, and three subsets of colors $C^{\inn},C^{\out},C^{\sib} \subseteq C$. A (partial) consistent subset of the subtree $T_i(v)$ with respect to the parameters $d^{\inn}$, $d^{\out}$, $d^{\sib}$, $C^{\inn}$, $C^{\out}$, $C^{\sib}$ is defined as a set of vertices $W\subseteq V(T_i(v))$ such that for any arbitrary subset $X\in \Esib(v,d^{\sib},C^{\sib})$ and $Y\in\Eout(v,d^{\out},C^{\out})$ (assuming they exist), $W$ satisfies the following (see Figure~\ref{fig:tree}): 

\begin{mdframed}[backgroundcolor=red!10,topline=false,bottomline=false,leftline=false,rightline=false] 
\begin{itemize}
    %\setlength{\parskip}{0pt}
    %\setlength{\itemsep}{0pt plus 1pt}
    \item $d(v,W)=d^{\inn}$. {(i.e., the distance of $v$ to its nearest member(s) in $W$ is $d^{\inn}$)}
    \item $C(\NN(v,W))=C^{\inn}$. {(i.e., $C^{\inn}$ is the set of colors of the nearest members of $v$ in the set $W$} 
    \item For every vertex $u\in T_i(v)$, $C(u)\in C(\NN(u,W\cup X\cup Y))$. 
\end{itemize}
\end{mdframed}\label{def1}
\end{definition}

Note that for some values of $d^{\inn},d^{\out},d^{\sib},C^{\inn}, C^{\out},C^{\sib}$ there may not exist any (partial) consistent subset for $T_i(v)$, in such a case we define it to be undefined. Also note that, for some values, the (partial) consistent subset can be empty as well, such as when $d^{\inn}= \infty$ and $C(u)\in C(\NN(u, X\cup Y))$ for every vertex $u\in T_i(v)$. For ease of notation, we will denote a (partial) consistent subset for $T_i(v)$ as a consistent subset with respect to the parameters $d^{\inn},d^{\out},d^{\sib},C^{\inn}, C^{\out},C^{\sib}$. %\red{$CCS(T_i(v))$}. \blue{Aritra: then we have to define it as  $CCS(T_i(v),d^{\inn},d^{\out},d^{\sib},C^{\inn}, C^{\out},C^{\sib})$}

%\red{{\bf Question:} Whether such a $W$ always exists?}
%For any vertex $v$, we use $T_{i}(v)$ to denote the union of sub-trees corresponding to the first $i$ children, i.e., $T_{i}(v)=\cup_{1\leq j\leq i} T(v_j)$. The union of sub-trees corresponding to the other children of $v$ is $T_{i+}(v) = \cup_{i+1\leq j\leq \eta_v} T(v_j)$. 

%\todo{write $\cap_{i+1\leq j\leq \eta_v} T(vj)$ by $T_{i+}(v)$. }







\begin{figure}[h]
                \centering
                \includegraphics[scale=0.7]{tree1}
                \caption{$\blacksquare$ vertices denotes consistent subset. $\dinvs=1,\doutvs=2,\dsibvs=1$}
                \label{fig:tree}
\end{figure}


%We design a bottom-up dynamic programming that runs from leaves up to the root. The idea is to compute a minimum consistent subset for $T_{i}(v)$ \todo{define min consistent subset for a subtree} with some (constant many) assumptions about the minimum solution for the rest of the tree. 

%\vspace{-\topsep}
% \begin{itemize}
%     %\setlength{\parskip}{0pt}
%     %\setlength{\itemsep}{0pt plus 1pt}
%     \item [ $\dinvs$:] Distance from $v$ to the closest vertex in $\svin$.
%     \item [ $\cinvs$:] Colors of the set of vertices in $\svin$ that are at distance $\dinvs$ from $v$.
%     \item [ $\dsibvs$:] Distance from $v$ to the closest vertex in $\svsib$.
%     \item [ $\csibvs$:] Colors of the set of vertices in $\svsib$ that are at distance $\dsibvs$ from $v$.
%     \item [ $\doutvs$:] Distance from $v$ to the closest vertex in $\svout$.
%     \item [ $\coutvs$:] Colors of the set of vertices in ${\overline{v}}$ that are at distance $\dsibvs$ from $v$.
% \end{itemize}

Consider an arbitrary consistent subset $S_T$ of $T$, an arbitrary vertex $v\in V(T)$ and an integer $i\in[\eta_v]$ (see Figure~\ref{fig:tree}).
%Now, consider the consistent subset $S_T$ for $T$ . 
For any vertex $v\in V(T)$ and $1\leq i\leq \eta_v$, define  
$\svin=S_T\cap V(T_i(v))$, $\svsib=S_T\cap V(T_{i+}(v))$, and $\svout=S_T\cap V(T\setminus T(v))$. Also define $\dinvs =d(v,\svin)$, $\cinvs= C(\NN(v,\svin))$, $\dsibvs=d(v,\svsib)$, $\csibvs=C(\NN(v,\svsib))$, $\doutvs =d(v,\svout)$, $\coutvs= C(\NN(v,\svout))$. Let $W$ be any arbitrary (partial) consistent subset with respect to the parameters $\dinvs,\doutvs,\dsibvs,\cinvs,\coutvs,\csibvs$ (see Definition \ref{def1}). Next we have the following lemma.
   
% For any arbitrary value of $v\in V(T)$,  $i\in[\eta_v]$, $0\leq \dinv\leq n$, $1\leq \doutv,\dsibv \leq n$, and $\cinv,\coutv,\csibv \subseteq C$ let us define  the following.
% Let $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$ denotes an aribitrary subsets of $V(T_i(v))$ such that the following properties holds.


% \begin{mdframed}[backgroundcolor=red!10,topline=false,bottomline=false,leftline=false,rightline=false] 

% \noindent{\bf Properties:}
% \begin{enumerate}\label{prop:DP}
%     \item The closest vertex in $P$ from $v$ is at distance $\dinv$, i.e. $\dinv=d(v,P)$.
%     \item Vertices in $P$ that are at distance $\dinv$ from $v$ is of color $\cinv$.
    
%     \item There is a set of vertex $X$ in $T_{i+}(v)$ at distance  $\dsibv$ from $v$ of color $\csibv$.
    
%     \item There is a set of vertex $Y$ in $T-T_v$ at distance  $\doutv$ from $v$ of color $\coutv$.
%     \item $P\cup X\cup Y$ is a consistent subset for $T_{i}(v)$ that is for all $v\in T(v), C(\NN(v,P\cup X\cup Y))=C(v)$.

% \end{enumerate}
% \end{mdframed}



\begin{lemma}
    $S_W=(S_T\setminus \svin)\cup W$ is a consistent subset for $T$. \label{claim:DP}
\end{lemma}

\begin{proof}

% Observe that if $S_T$ is a consistent subset of $T$, then $S$ can be written as $A\cup B$, $A$ and $B$ not necessarily disjoint, such that the nearest neighbor of the same color in $S_T$ of a vertex $u$ in $T_i$ lies in $A$  the nearest neighbor of the same color in $S_T$ of a vertex $w$ in $T\setminus T_i(v)$ lies in $B$. For an arbitrary choice of $A$ and $B$, if no vertex in $A$ is nearest to a vertex in $T\setminus T_i(v)$ and no vertex in $B$ is nearest to a vertex in $T_i$, then $S_T$ is a consistent subset of $T$. From Figure~\ref{fig:tree}, one such choices of $A$ and $B$ are, $A=S\setminus \svin \cup \NN(v,\svin)$ and $B=\svin\cup \NN(v,\svsib) \cup \NN(v,\svout)$. 

 
Suppose that $A= W\cup \NN(v,\svsib) \cup \NN(v,\svout)$  is the set of vertices which are either in $W$ or in the nearest neighbor of $v$ outside $T_i(v)$ in $S_W$. We will show that for any vertex $u\in T_i(v)$, $NN(u,S_W)\subseteq A$ and there is a vertex in $NN(u,A)$ of the color same as $u$. Similarly, let $B=(S_W\setminus W) \cup \NN(v,W)$. We show that for any vertex $w$ outside $T_i(v)$, $NN(w,S_W)\subseteq B$ and there is a vertex in $NN(w,B)$ of the color same as  $w$. Please note that $A$ and $B$ are not necessarily disjoint.
%, such that any vertex $u$ in $T_i$ has a nearest neighbor of the same color in $A$ and any vertex $w$ in $T\setminus T_i(v)$ has a nearest neighbor of the same color in $B$. For one such choice of $A$ and $B$, 
%if no vertex in $A\setminus B$ is nearest to a vertex in $T\setminus T_i(v)$ and no vertex in $B \setminus A$ is nearest to a vertex in $T_i$, then $S_T$ is a consistent subset of $T$. From Figure~\ref{fig:tree}, if $A=S\setminus \svin \cup \NN(v,\svin)$ and $B=\svin\cup \NN(v,\svsib) \cup \NN(v,\svout)$, then $A\cup B=S_T$ forms a consistent subset of $T$.

%Let $S=S_T\setminus \svin\cup W$. $S$ can also be written as $A\cup B$ with  $A= W\cup \NN(v,\svsib) \cup \NN(v,\svout)$ and $B=S\setminus \svin \cup \NN(v,W)$. 
Consider a vertex $u\in T_i(v)$ and  $w \in T\setminus T_i(v)$. Since $\NN(v,\svsib)\in \Esib(v,\dsibvs,\csibvs)$, $\NN(v,\svout) \in \Eout(v,\doutvs,\coutvs)$, and $W$ is a consistent subset with respect to the parameters $\dinvs,\doutvs,\dsibvs,\cinvs,\coutvs,\csibvs$,  we have $C(u)\in C(\NN(u,W\cup \NN(v,\svsib) \cup \NN(v,\svout)))= C(\NN(u,A))$. Also, as $S_T$ is a consistent subset, we have $C(w)\in C(\NN(w, S_T\setminus \svin)\cup \cinvs$. From the properties of $W$, we have $C(\NN(v,W))=\cinvs$. Hence, $C(w)\in C(\NN(w, B))$. Thus to prove the result, it is enough to show that (i) no vertex from $B\setminus A$ can be the closest to the vertex $u$ in the set $S_W$, and (ii) no vertex from $A\setminus B$ can be the closest vertex of $w$ in the set $S_W$.  We prove these two claims by contradiction. 

Let \textit{Claim (i)} be false. Then, there will be a vertex $x\in B\setminus A$, which is closest to $u$. Note that, $(B\setminus A)\cap ((T_i(v)\cup \NN(v,\svsib) \cup \NN(v,\svout))= \emptyset$. Hence we have, $d(u,x)=d(u,v)+d(v,x)$, $d(v,x)>min(\dsibvs,\doutvs)$. This is a contradiction as the closest vertex from $v$ in $S_W \cup (T\setminus T_i(v))$ (if it exists) is at distance $min(\dsibvs,\doutvs) =d(v,\NN(v,\svsib) \cup \NN(v,\svout))$. Hence, $x$ cannot be the closest vertex of $u$ in $S_W$. Thus, \textit{Claim (i)} follows.
% contradiction as $min(\dsibvs,\doutvs)=d(v,\NN(v,\svsib) \cup \NN(v,\svout))$ and the closest in $T\setminus T_i(v) $ from $v$ (if it exists is a vertex at this distance. Hence, $x$ cannot be the closest vertex of $u$ in $S_W$. Thus, \textit{Claim (i)} follows. 

Now, let \textit{Claim (ii)} be false. Then there is a vertex $y \in A\setminus B$, which is closest to $w$. As $w \not\in T_i(v)$ and $y \in T_i(v)$, we have $d(w,y)=d(w,v)+d(v,y)$. Since $d(v,\NN(v,W))=\dinvs$ and $w\in (A\setminus B = W\setminus \NN(v,W))$, we have $d(v,y)>\dinvs$. This contradicts the fact that the closest vertex from $v$ in $S_W \cup T_i(v)$ (if it exists) is at distance $\din$ from $v$. Hence \textit{Claim (ii)} is true.
\end{proof} 




% \begin{lemma}
%     $(S_T\setminus \svin)\cup W$ is a consistent subset for the tree $T$.  \label{claim:DP}
% \end{lemma}

% \begin{proof}
% Let $S=(S_T\setminus \svin)\cup W=A\cup B$ (say), where $A= W\cup \NN(v,\svsib) \cup \NN(v,\svout)$ and $B=(S\setminus \svin) \cup \NN(v,W)$ \red{(Please check the definition of $B$. If so, then check the proof of Claim (i))}. To show, $S$ is a consistent subset. Consider an arbitrary vertex $u\in T$. Here, two cases need to be considered: (i) $u \in T_i(v)$, and (ii) $u \in T\setminus T_i(v)$. In Case (i), since $\NN(v,\svsib)\in \Esib(v,\dsibvs,\csibvs)$ and $\NN(v,\svout) \in \Eout(v,\doutvs,\coutvs)$, we have $C(u)\in C(\NN(u,W\cup \NN(v,\svsib) \cup \NN(v,\svout)))= C(\NN(u,A))$. In Case (ii), consider the fact that $S_T$ is also a consistent subset. So, we have $C(u)\in C(\NN(u,S_T\setminus \svin)\cup \cinvs$. From the properties of $W$, we have $C(\NN(v,W))=\cinvs$. Hence, $C(u)\in C(\NN(u, B))$. Therefore, it is enough to show that 

% \begin{description}
% \item[Claim (i)] none of the vertices of $B$ ($\subset S$) can be closest to any vertex in $T_i(v)$, and 
% \item[Claim (ii)] none of the vertices in $A$ ($\subset S$) can be closest to any vertex in $T\setminus T_i(v)$.
% \end{description}

% Let \textit{Claim (i)} be false. Then, there is a vertex $u\in T_i(v)$ whose closest vertex in $S$ is a vertex $x\in B (=S\setminus A)$. Note that $B\cap (T_i\cup \NN(v,\svsib) \cup \NN(v,\svout))= \emptyset$ (from the definition of set $B$ \red{(Why? $B$ contains $NN(v,W)$, and $W$ contains members of $T_i$.)}).
% %$(S\setminus A)\cap (T_i\cup \NN(v,\svsib) \cup \NN(v,\svout))= \emptyset$. 
% Hence we have, $d(u,x) = d(u,v)+d(v,x)$ and $d(v,x)>min(\dsibvs,\doutvs)$. This is a contradiction as $min(\dsibvs,\doutvs)=d(v, \NN(v,\svsib) \cup \NN(v,\svout))$ and there is a vertex at this distance. Hence, $x$ can not be the closest to the vertex $u$ in the set $S$. 



% If \textit{Claim (ii)} is false, then there is a vertex $y$ in $S\setminus B$ which is closest to $u\in T\setminus T_i(v)$, implying $d(u,y)=d(u,v)+d(v,y)$. Since $d(v,\NN(v,W))=\dinvs$ and $u\in (S\setminus B = W\setminus \NN(v,W))$, $d(v,y)>\dinvs$. This is a contradiction as there is a vertex in $S$ at distance $\din$ from $v$ and \textit{Claim 2} is true.

% Thus, the proof of the lemma follows.  
% \end{proof}

% We know from the previous properties, $A$ is a consistent subset for $T_i(v)$. Suppose the \textit{claim 1} is not true. In that case, there is a vertex $x \in S\setminus A$ that is closest to $u$. Let $d(u,x)$ be the distance between $u$ and $x$. Observe that $d(u,x)=d(u,v)+d(v,x)$ and $d(v,x)> min (\dsibvs,\doutvs)$. This is a contradiction as there are vertices in $S$ at distance $min(\dsibvs,\doutvs)$. Hence, \textit{claim 1} is true. 


% Similarly, let $w$ be a vertex in $T\setminus T_i(v)$. 

% \textit{Claim 2:} The closest vertex from $w$ in $S$ lies in $B= S \setminus P(T_{i}(v),\dinvs,\doutvs,\dsibvs,\cinvs,\coutvs,\csibvs) \cup Z$. Where $Z$ is the set of vertices in $S\cap T_i(v)$ at distance $\dinvs$ of colour $\cinvs$. 

% Observe that such set $Z$ exists since $P(T_{i}(v),\dinvs,\doutvs,\dsibvs,\cinvs,\coutvs,\csibvs)$ contains vertices at distance $\dinvs$ of colours $\cinvs$. Correctness of \textit{claim 2} can be proved in a ma\NNer similar to that of \textit{claim 1}. The closest vertices in $B$ from $W$ are the same as the closest vertices in $S_T$ from $w$. So, $B$ forms a consistent subset of $T\setminus T_i(v)$.

% Set $S$ can also be written as $A\cup B$ with $A\cap B = X\cup Y\cup Z$. From \textit{claim 1} and \textit{claim 2}, $A\cup B $ will not affect the consistency for $T_i(v)$ (similarly for $T\setminus T_i(v)$) and every vertex in $T$ will have a nearest neighbour of the same color. Hence, $S$ is a consistent subset of $T$.
%\end{proof}


Motivated by Lemma \ref{claim:DP}, we design the following algorithm based on dynamic programming technique. For each choice of $v\in V(T)$, $i\in[\eta_v]$, $\dinv \in [n] \cup \{0,\infty\}$, $\doutv \in [n]\cup \{\infty\}$, $\dsibv \in [n]\cup \{\infty\}$, and $\cinv,\coutv,\csibv \subseteq C$, we define a subproblem which computes the cardinality of a minimum sized (partial) consistent subset for the subtree $T_i(v)$ with respect to the parameters $\langle \dinv,\doutv,\dsibv,\cinv,\coutv,\csibv \rangle$, and %We denote the consistent subset by $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$.
denote its size by $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$.
% A consistent subset for a subtree
% % For a node $v$, let $T(v)$ be the sub-tree rooted at $v$.
% Each subproblem computes an arbitrary subset $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$.
Let us use $\dminv=\min(\dinv,\doutv,\dsibv)$.
\begin{align*}
  A = 
  \begin{cases}
    \cinv  \textrm{ if  }\dinv=\dminv,\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
  &B = 
  \begin{cases}
    \csibv \textrm{ if  }\dsibv= \dminv,\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
  &D = 
  \begin{cases}
    \coutv  \textrm{ if  }\doutv= \dminv,\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
\end{align*}

We define $\cminv=A\cup B\cup D$.

Note that $\dminv$ is the distance of the closest vertex to $v$ in the consistent subset, and $\cminv$ denotes the colors of all such vertices. 

To compute any DP entry, we take into account the following six cases. The first two cases are for checking whether a DP entry is valid. The third case considers the scenario in which $v$ is part of the solution; the fourth, fifth, and sixth cases collectively consider the scenario in which $v$ is not in the solution


% , and 

% $\cminv=\{\cup_x C_v^{x} | x\in \{\inn,\out,\sib\} \textrm{ and } \delta_v^x=\dminv\}$.%  \textrm{ and } \delta_v^x=\dminv \red{???} \} $ 

\begin{figure}[t]
                \centering
                \includegraphics[scale=1.3]{dp1}
                \caption{Illustration of the Case 3, where $\dinv=0$}
                \label{fig:dpatv}\vspace{-0.2in}
\end{figure}


\begin{description}
\item[Case 1:] If $C(v) \notin \cminv$, return $\infty$. 
        %\red{What is $C(v)$? As I can see, it is not defined.}

\item[Case 2:] $\dinv=0$ and $\cinv\neq\{C(v)\}$. Here, return $\infty$.

\item[Case 3:] $\dinv=0$ and  $\cinv=\{C(v)\}$. Here,  return  $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)=$
    $$ 1+\sum_{1\leq j\leq i} 
    \biggl\{ \min_{\delta,C'} 
    P\Bigl(T_{\eta_{v_j}}(v_j),\delta,1,\infty,C',\{C(v)\},\emptyset\Bigr)
    \biggr\}
    $$
\end{description}

\noindent {\bf Explanation:} Case 1 and Case 2 are self-explanatory. Case 3 implies that the vertex $v$ is included in the consistent subset. Consequently, for the optimal solution, we need to determine a consistent subset for each tree rooted at a child $v_j$ of $v$, independently of each other, assuming that $v$ is part of the consistent subset (refer to Figure~\ref{fig:dpatv}). For every child $v_j$ of $v$, we iterate through all possible choices of $C'\subseteq C$ and $\delta^{\inn}_{v_j}=\delta\in \{1, \ldots, h(T(v_j)\}\cup \{\infty\}$ where $h(T(v_j))$ is the height of the tree rooted at $v_j$, to identify the minimum consistent subset for $T_{\eta_{v_j}}(v_j)$. This is done with the constraints that the closest vertex in the consistent subset inside $T_{\eta_{v_j}}(v_j)$ is at a distance $\delta$ and spans $C'$. For any vertex in $T(v_j)$, the path of the closest vertex of its own color outside $T_i(v)$ has to pass through $v$, which is considered to be in the consistent subset and has color $C(v)$. Thus, $\doutv=1$ is taken for the tree $T_{\eta_{v_j}}(v_j)$. Since we are solving for the complete tree rooted at $v_j$ with no siblings, we set the distance to the closest sibling vertex as $\dsibv=\infty$ and the corresponding color set as $\emptyset$.

In the rest of the section, we consider three more cases where $\dinv>0$, and hence $\dinv,\doutv,\dsibv>0$. Intuitively, while solving the problem recursively, we will recursively solve $\mcs$ in $T_{i-1}(v)$ and $T_{\eta_{v_i}}(v_i)$. We try all possible sets of choices of $C_a, C_b$ with $\cinv=C_a\cup C_b$, and recursively solve for a solution assuming that the nodes of colors in $C_a$ are present in $T_{i-1}(v)$ at distance $\dinv$ (if $C_a\neq\emptyset$ and such choices are feasible) and nodes of colors in $C_b\subseteq\cinv$ are present in $T_{\eta_{v_i}}(v_i)$ at distance $\dinv-1$ from $v_i$ (if $C_b\neq\emptyset$ and such choices are feasible). 


Note that in the following case, the closest colored vertices in the consistent subset from $v$ in both $T_{i-1}(v)$ and $T_{\eta({v_i})} (v_i)$ are located at a distance of precisely $\dinv$

\begin{description}
\item[Case 4:] $C_a,C_b\neq \emptyset$. %\red{(We are dealing with the case where $\dinv>0$; does it need to be explicitly written here? It is mentioned in the previous paragraph)}


We define the following. Let $\delta_x = \min(\dinv,\dsibv)$ and $\delta_{\min}=\min(\dinv,\dsibv,\doutv)$. 




\begin{align*}
C_{i-1}^{\sib} &= 
  \begin{cases}
    C_b & \textrm{ if  }\dinv< \dsibv \textrm{ and  } C_b\neq \emptyset ,\\
    C_b \cup \csibv & \textrm{ if  }\dinv= \dsibv,\\
    \csibv & \text{ otherwise },
  \end{cases}
  % & X &= 
  % \begin{cases}
  %   \C_b  \textrm{ if  }\dinv= \delta_{\min},\\
  %   \emptyset \textrm{ Otherwise  },
  % \end{cases}
\end{align*}
Here $\delta_x$ is the distance of the closest vertices in the consistent subset from $v$ that lies in $T_{(i-1)+}(v)$ and $C_{i-1}^{\sib}$ is the color set of those vertices. Hence they function as the distance of closest vertices (and their colors) in the consistent subset that lies in the sibling branches of $v$ for the tree $T_{(i-1)}(v)$. %Similarly, $\delta_{min} + 1$, is the distance of closest vertex from $v_i$ in the consistent subset for $T_{\eta(v_i)} (v_i)$ and $C$ i is the set of corresponding colors.
Also, define $C_i^{\out}=A\cup B\cup D$, where

\begin{align*}
  A = 
  \begin{cases}
    \C_a  \textrm{ if  }\dinv= \delta_{\min},\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
  &B = 
  \begin{cases}
    \csibv \textrm{ if  }\dsibv= \delta_{\min},\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
  &D = 
  \begin{cases}
    \coutv  \textrm{ if  }\doutv= \delta_{\min},\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
\end{align*}

\begin{figure}[h]
                \centering
                \includegraphics[scale=1.4]{dp2}
                \caption{Illustration of the Case 4}
                \label{fig:dpnonempty}
\end{figure}

%If $C_a,C_b\neq \emptyset$, 
\begin{tabbing}
Return $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$\= = $\displaystyle{\min_{C_a,C_b} \Bigl( P\Bigl( 
        T_{i-1}(v),\dinv,\doutv,\delta_x,C_a ,\coutv,C_{i-1}^{\sib} 
        \Bigr) +}$ \\
\> $\displaystyle{P\Bigl(
        T_{\eta_{v_i}}(v_i),\dinv-1,\delta_{\min}+1,\infty,C_b, C_i^{\out}, \emptyset
        \Bigr) \Bigl)}$
\end{tabbing}        
\end{description}

\noindent {\bf Explanation:} In this case we iterate over all possible choices of $C_a$ and $C_b$, assuming $C_a, C_b\neq \emptyset$ and $C_a\cup C_b=\cinv$. In the first part of the recursive formula, we recursively solve the problem for the tree $T_{i-1}(v)$ with the restriction that we have to include a set of vertices of color $C_a$ in $T_{i-1}(v)$ at distance $\dinv$ from $v$ (see Figure~\ref{fig:dpnonempty})  Restriction on $\coutv$ and $\doutv$ among the vertices in $T\setminus T(v)$ remain same as that of the parent problem. Regarding $\csibv$ and $\dsibv$,  observe that vertices in $T(v_i)$ and $T_{i+}$ are part of $T_{(i-1)+}$. Therefore the parameters for the sibling depend on the value of $\dinv$ and $\dsibv$, and accordingly, we have defined $C_{i-1}^{\sib}$.

In the second part of the recursive formula, we are solving the problem recursively for the tree $T_{\eta_{v_i}}(v_i)$, with the restriction that, in the consistent set in the consistent set we have to include a set of vertices from $T_{\eta_{v_i}}(v_i)$ which are of colors $C_b$, and at distance $\dinv-1$ from $v_i$. Observe that the vertices in $T_{i-1}(v)$, $T_{i+}(v)$ and $T\setminus T(v)$ are all outside $T(v_i)$. Thus the restriction on the distance to the vertices on the consistent subset outside $T(v_i)$ and their colors depend on the values of $\dinv,\dsibv$ and $\doutv$. Thus the distance $\doutv$ of this subproblem is defined as $\delta_{\min}=\min(\dinv,\dsibv,\doutv)$, and the set of colors $C_i^{\out}$ is defined accordingly. As we are solving for the whole tree rooted at $v_i$, there are no siblings; so $\dsibv=0$ and $C_i^{\sib}=\emptyset$.


\begin{description}
\item[Case 5:] $C_a=\emptyset$ and $C_b=\cinv$.

Observe that in this case, the closest vertex in the consistent subset in $T_{i-1}(v)$ should be at a distance at least $\dinv+1$. We iterate over all values $\delta>\dinv$ and all possible choices of colors to find the size of a minimum consistent subset. 
We define $\delta_x$ and $C_{i-1}^{\sib}$ same as in Case 4. 
For any values $\delta>\dinv$ and $C\subseteq [c]$, we define $\delta_{\min}(\delta,C)=\min(\delta,\dsibv,\doutv)$, and $C_i^{\out}(\delta,C)=A\cup B\cup D$ where
\begin{align*}
  A = 
  \begin{cases}
    \C  \textrm{ if  }\delta= \delta_{\min},\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
  &B = 
  \begin{cases}
    \csibv \textrm{ if  }\dsibv= \delta_{\min},\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
  &D = 
  \begin{cases}
    \coutv  \textrm{ if  }\doutv= \delta_{\min},\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
\end{align*}



\begin{tabbing}
Return $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$ \= =  $
\displaystyle{\min_{\delta>\dinv,C\subseteq [c]}\Bigl( P\Bigl( 
        T_{i-1}(v),\delta,\doutv,\delta_x,C ,\coutv,C_{i-1}^{\sib} 
        \Bigr)} + $\\
\>$\displaystyle{P\Bigl(
        T_{\eta_{v_i}}(v_i),\dinv-1,\delta_{\min}(\delta,C)+1,\infty,C_b, C_i^{\out}(\delta,C), \emptyset
        \Bigr)\Bigl)}$
\end{tabbing}
\end{description}

\noindent {\bf Explanation:} It is the same as Case 4 except for the fact that we have to make sure that the closest vertex chosen in the consistent subset from $T_{i-1}(v)$ is at distance at least $\dinv+1$.

\begin{description}
\item[Case 6:] $C_b=\emptyset$ and $C_a=\cinv$.

Next, we consider the case when $C_b=\emptyset$ and $C_a=\cinv$. 
$\delta_{\min}(\delta,C)=\min(\dinv,\dsibv,\doutv)$. We define $C_i^{\out}(\delta,C)=A\cup B\cup D$ where
\begin{align*}
  A = 
  \begin{cases}
    \C_a  \textrm{ if  }\dinv= \delta_{\min},\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
  &B = 
  \begin{cases}
    \csibv \textrm{ if  }\dsibv= \delta_{\min},\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
  &D = 
  \begin{cases}
    \coutv  \textrm{ if  }\doutv= \delta_{\min},\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
\end{align*}

For any values $\delta>\dinv$ and $C\subseteq [c]$ we define
$\delta_x(\delta,C)=\min(\dsibv,\delta)$ We define $C_{i-1}^{\sib}(\delta,C)=E\cup F$ where
\begin{align*}
  E = 
  \begin{cases}
    \C  \textrm{ if  }\delta= \delta_x(\delta,C),\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
  &F = 
  \begin{cases}
    \csibv \textrm{ if  }\dsibv= \delta_x(\delta,C),\\
    \emptyset \textrm{ Otherwise  }
  \end{cases}
\end{align*}


Return $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$ =
%\begin{multline*}

$\displaystyle{
\min_{\delta>\dinv,C\subseteq [c]}\Bigl(P\Bigl( 
        T_{i-1}(v),\dinv,\doutv,\delta_x(\delta,C),C_a ,\coutv,C_{i-1}^{\sib}(\delta,C) 
        \Bigr) + 
        P\Bigl(
        T_{\eta_{v_i}}(v_i),\delta,\delta_{\min}+1,\infty,C_b, C, \emptyset
        \Bigr)}\Bigl)$
%\end{multline*}
\end{description}
\noindent {\bf Explanation:} It is the same as the previous two cases.

% \red{KP: (case 3,4 and 5 doesn't give $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$, $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$ should be min (case 3, case 4, case 5)) }


% For all possible choices of $C_a$ and $C_b$ such that $\cinv=C_a\cup C_b$, we compute the following. we define 
% % \begin{equation*} \label{eq1}
% % \begin{split}
% % \delta_x & = \dinv \textrm{ if  }\dinv\leq \dsibv \textrm{ and  } C_b\neq \emptyset\\
% %  & = \dsibv \textrm{ otherwise  }
% % \end{split}
% % \end{equation*}


 
% \begin{align*}
% \delta_x &= 
%   \begin{cases}
%     \dinv & \textrm{ if  }\dinv\leq \dsibv \textrm{ and  } C_b\neq \emptyset ,\\
%     \dsibv & \text{ otherwise },
%   \end{cases}
%   & \delta_u &= 
%   \begin{cases}
%     \dinv & \textrm{ if  }\dinv\leq \dsibv \textrm{ and  } C_a\neq \emptyset ,\\
%     \dsibv & \text{ otherwise },
%   \end{cases}
%   \\
% \C_x &= 
%   \begin{cases}
%     \C_b & \textrm{ if  }\dinv< \dsibv \textrm{ and  } C_b\neq \emptyset ,\\
%     \C_b \cup \csibv & \textrm{ if  }\dinv= \dsibv,\\
%     \csibv & \text{ otherwise },
%   \end{cases}
%   & \C_u &= 
%   \begin{cases}
%     \C_a & \textrm{ if  }\dinv< \dsibv \textrm{ and  } C_a\neq \emptyset ,\\
%     \C_a \cup \csibv & \textrm{ if  }\dinv= \dsibv,\\
%     \csibv & \text{ otherwise },
%   \end{cases}
% \end{align*}

% We define, 
% $P_a = P\Bigl( 
%         T_{i-1}(v),\delta_y,\doutv,\delta_x,C_y ,\coutv,C_x 
%         \Bigr)$ where, $\delta_y$  and $C_y$ are defined as follows.  If $C_a\neq \emptyset$ we define $\delta_y=\dinv$ $C_y=C_a$ otherwise, we choose  $\delta_y>\dinv$ and $C_y$ to be any arbitrary subset of the $k$ colours. %such that the cardinality of $P_a$ is minimized.
       

% We define $P_b$ as follows. 
% $P_b=P\Bigl(
%         T_{\eta_{v_i}}(v_i),\delta_v,\delta_z,\delta_u,C_v, C_z, C_u
%         \Bigr)$ where $\delta_v,C_v,\delta_z$ and $C_z$ are defined as follows.  If $C_b\neq \emptyset$ we define $\delta_v=\dinv-1$ and $C_v=C_b$ otherwise, we choose  $\delta_v>\dinv-1$ and $C_v$ to be any subset of $k$ colours such that the cardinality of $P_b$ is minimized.

%         For $\delta_z$ and $C_z$ we define $\delta_z=min\{\delta_y+1,\dsibv+1,\doutv+1\}$ and $C_z=\cup C_s$ where,$$C_s=\begin{cases}
%             C_y &\text{ if } \delta_z=\delta_y+1 \\
%             \cup_x C_v^{x} &\text{ if } \delta_z=\delta_v^x+1, x\in \{\out,\sib\}
%         \end{cases}$$
        
%         $\delta_y$ and $C_y$ are chosen such that the cardinality of $P_a \cup P_b$ is minimized.
        
% We have,  
% $$P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)=\min(P_a \cup P_b)$$.




\subsection*{Running time of the algorithm} 
The total number of choices of $\dinv,\doutv,\dsibv,\cinv,\coutv$ and $\csibv$ is bounded by $n^3 2^{3c}$. For each choice $C_a$ and $C_b$, the algorithm takes at-most $n2^c$ time to go through all possible entries of $\delta$ and $C$ (in \textbf{case 5} and \textbf{case 6}) and there are at-most $2^{2c}$ choices of $C_a$ and $C_b$. The recursion runs for at most $n^2$ times. Hence, the worst-case running time of the algorithm is $\mathcal{O}(2^{6c}n^6)$.



%For each subproblem along with the parameters  \vin, \vout, \vincol, \voutcol we introduce two other parameters, \vsib and  \vsibcol. \vsib denotes the distance to the closest vetrex in the \mcs inside the subtrees $T(ch_{i+2}(v))$, $T(ch_{i+3}(v))$, $\cdots T(ch_{c_v}(v))$ from $v$. \vsibcol denotes the colors of such vertices in the \mcs. At each stage, for the subtree $T_{i+1}(v)$ assuming that partial solutions for the subtree $T_i(v)$ is already computed, our algorithm computes a partial solution, 
% $$P(T_{(i+1)}(v),\delta_v^{IN},\delta_v^{OUT},\delta_v^{SIB},C_v^{IN},C_v^{OUT},C_v^{SIB})$$
% which returns a set $S$ of minimum cardinality such that $S\cup S^{OUT} \cup S^{SIB}$ is a consistent subset for $T_{(i+1)}(v)$, where $S^{OUT}$ is a set of vertices of colour \voutcol at a distance \vout and $S^{SIB}$ is a set of vertices of colour \vsibcol at a distance \vsib from $v$. 

%We denote the set of colors of the vertices in the consistant subset that are at distance \vin (or \vout) by \vincol (\voutcol respectively). As there can be multiple vertices in the consistant subset that are at distance \vin if we use the conventional dynamic programming approach used in the previous section, the solution for a subproblem defined by the tree rooted at $v$, may depend on $n_c^{|\textrm{\vincol}|}$ subproblems where $n_c$ be the number of children of $v$. To avoid this we define our subproblems as follows.















%$P$ is defined by the following parameters $T_{i}(v),\dinv,\doutv,\dsibv,\cinv,$ $\coutv,\csibv$. Here $v\in V(T)$,  $i\in[\eta_v]$, $0\leq \dinv\leq n$, $1\leq \doutv,\dsibv \leq n$, and $\cinv,\coutv,\csibv \subseteq C$ \todo{Define $C$ to be set of all colors}.
%Each $P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$ compute a minimum consistent subset $S$ for the vertices in $T_{i}(v)$ with the assumptions mentioned above. 
 
% For every vertex $v\in V(T)$ and every integer $i\in[\eta_v]$ we define the subproblem $P_i(v)$. Each subproblem $P_i(v)$ also depends on the following parameters 

% $$P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$$
%At each stage, our algorithm computes a \textit{partial solution} $P_i(v)$ for $T_i(v)$. Each subproblem 

%The \textit{partial solution} is a set of vertices that satisfy consistency for some of the vertices in $T_i(v)$.  

%We allow some vertices to remain unsatisfied but keep track of them.

 



% \textbf{Intuition:}
% While processing a vertex $v$, it maintains a parameter $\delta_v^x$, and an index $x$. For each $i =1,2,\ldots, \eta_v$, it considers $T_i(v)$, and computes $\dinv$ = the distance of node $v$ from the nearest vertex in \mcs inside $T_i(v)$, $\dsibv$ = 
% the distance to the nearest vertex in \mcs inside $T_{i+}(v)$, and $\doutv$ = the 
% distance to the nearest vertex in \mcs outside $T_{\eta_v+}(v)$ (i.e., $T\setminus T(v)$). The consistent subsets corresponding to these counts in $T_i(v)$, $T_{i+}(v)$ and in $T\setminus T(v)$ are denoted by $\cinv$, $\csibv$ and $\coutv$ respectively. It computes  $\dminv=\min(\dinv,\doutv,\dsibv)$, and then computes  $\cminv=\cup_{x\in \{\i\NN,\out,\sib\}} C_v^{x}$. Finally, it sets $\delta_v^x=\dminv$. 


% The subset of colours in the \mcs that are at distance $\dinv$, $\doutv$, and $\dsibv$ for $T_i(v)$, are denoted by $\cinv$, $\coutv$ or $\dsibv$ respectively. \red{(Moreover, for different $T_i(v)$, do we have different $\dinv$? If so, how you can justify the routing $P$, written below?)} \todo{you can write along with these distances we also store the color information of facilities exactly at these distances that are desired in an optimal solution }

% For each $1\leq i\leq \eta_v$ our objective is to compute 

% $$P(T_{i}(v),\dinv,\doutv,\dsibv,\cinv,\coutv,\csibv)$$

% \red{WHAT is P? Is it the name of a routine?}
% \todo{So and Ss contains some vertices that are at this distance but may contain more}
% which returns a set $S$ of minimum cardinality such that $S\cup S_o \cup S_s$ is a consistent subset for $T_{i}(v)$, where $S_o$ is a set of vertices of colour $\coutv$ at a distance $\doutv$ and $S_s$ is a set of vertices of colour $\csibv$ at a distance $\dsibv$ from the node $v$. \red{What is $S$?}

==> Notations.tex <==
\section{Notation and Preliminary Results}
{\bf Notations.} Without loss of generality, we will use $[n]$ to denote the set of integers $\{1,\ldots, n\}$. For any graph $G$, we denote the set of vertices of $G$ by $V(G)$ and the set of edges by $E(G)$. For any two vertices $u,v \in V(G)$, we use $d(u,v)$ to denote the shortest path distance (number of edges in the shortest path) between $u$ and $v$ in $G$. For any graph $G$ and any vertex $v\in V$ let $N(v)=\{u|u\in V, (u,v)\in E\}$ denotes the set of neighbours of $v$ and $N[v]=\{v\}\cup N(v)$.  We denote the distance between two subgraphs $G_1$ and $G_2$ in $G$ by $d(G_1,G_2)=\min \{d(v_1,v_2)|v_1\in V(G_1),v_2\in V(G_2)\}$. For any subset of vertices $U\subseteq V$ in a graph $G$, $G[U]$ denotes the subgraph of $G$ induced on $U$. Most of the symbols and notations of graph theory used are standard and taken form \cite{diestel2012graph}. 

%\subsection{log APX approximation for \mcs}


As an elementary result, we prove that \mcs is \lapxh.
We reduce the dominating set problem to the consistent subset problem (\csp). In the {\em dominating set problem} given a graph $G$ and an integer $k$ the objective is to find out whether there exists a subset $U\subseteq V$ of size $k$ such that for any vertex $v\in V$, $N[v]\cap U\neq \emptyset$. It is known that the Set Cover problem is \lapxh, or in other words, it is $\nph$ to approximate the Set Cover problem within a $c\cdot \log n$
 factor~\cite{raz97}. As there exists an $L$-reduction from set cover to dominating set problem, the dominating set problem is known to be \lapxh.
Let $(G,k)$ be any arbitrary instance of the dominating set problem with a graph $G$ and an integer $k$. We construct an instance $(H, C, k+1)$ of \csp as follows.
$V(H)=V(G)\cup\{x\}$ and $E(H)=E(G)\cup \{(x,v)|v\in V(G)\}$. For all $v \in V(G)$, We set $C(v)=1$, and set $C(x)=2$. 
% Now, we have the following lemma.
For the sake of completeness, we state the following known lemma with proof.

\begin{lemma}
    There exists a dominating set for $G$ of size at most $k$ if and only if there is a consistent subset of size at most $k+1$ for the graph $H$.\label{bubailemma6}
\end{lemma}
\begin{proof}
    Let $D$ be a dominating set of size $k$ for the graph $G$. We claim that $D'=\{x\}\cup D$ is a consistent subset of $H$. If not, then there be a vertex $v_i\in V(H)\setminus D'$ such that $d(v_i,D)>d(v_i,x)=1$. This contradicts that $D$ is a dominating set for $G$ and the claim holds.

    On the other hand, suppose $D'$ is a consistent subset of size $k+1$ in the graph $H$. Observe that $x\in D'$ as $x$ is the only vertex with color $2$. We claim that $D=D'\setminus \{x\}$ is a dominating set of $G$. If not, then there is a vertex $v\in V(G)\backslash D$ such that $N(v)\cap D=\emptyset$. Thus $d(v,D')>1$ but $d(v,x)=1$ and $C(v)\neq C(x)$. It contradicts the assumption that $C$ is a consistent subset and hence the claim holds.
\end{proof}
From Lemma~\ref{bubailemma6}, we have the following theorem.
\begin{theorem}
    There exists a constant $c>0$ such that it is $\nph$ to approximate the Minimum Consistent Set problem within a factor of $c\cdot \log n$.
\end{theorem}

 % \subsubsection{Reduction}
% Let $G(V, E)$ be a simple graph where $V=\{a_1,\dots, a_n\}$ and $E=\{e_1,\dots, e_m\}$. The reduction is as follows.
% \begin{enumerate}
%     \item For each vertex $a_i$ of $V$, we introduce a \emph{blue} vertex $b_i\in V^{'}$. Therefore $V^{'}$ has a total of $n$ \emph{blue} vertices.

%     \item Introduce a red vertex $r_1\in V^{'}$. Therefore Therefore $V^{'}$ has a total of $n+1$ vertices.

%     \item If $a_i$ and $a_j$ are adjacent in $E$, then the corresponding vertices $b_i$ and $b_j$ are adjacent in $E^{'}$. 

%     \item For each \emph{blue} vertex $b_i$ in $V^{'}$, we introduce an edge $b_ir_1$. Hence $E^{'}$ has a total of $m+n$ edges.

% \end{enumerate}
% \subsubsection{Properties of reduced graph}



% \begin{lemma}{\label{bubailemma6}}
%     A dominating set of $G(V,E)$ has $k$ vertices if and only if $G^{'}(V^{'},E^{'})$ has a consistent subset of size $k+1$.

    
% \end{lemma}

% \begin{proof}

%   Suppose a dominating set $D$ of the graph $G(V, E)$ has $k$ vertices. Without loss of generality, let the set $D$ be $\{a_1, a_2, \dots, a_k\}$. We claim that $C=\{r_1, b_1, b_2, \dots, b_k\}$ is a consistent subset of $G^{'}(V^{'}, E^{'})$. If not, then there be a vertex $b_i\in V\backslash C$ such that the distance of $b_i$ to the nearest vertex $b_j$ in $C$ is greater than one because $dist(b_i, r_1)=1$. Therefore the vertex representing of $b_i$ and $b_j$ in $G(V, E)$ must satisfies the the inequality $dist(a_i,a_j)>1$ where $a_j\in D$ and $a_i\notin D$. Hence $D$ is not a dominating set, a contradiction.
%    $\\ \\$
%    Suppose $C$ is a consistent subset of size $k$ in the graph $G^{'}(V^{'}, E^{'})$. Without loss of generality, let the set $C$ be $\{r_1, b_1, b_2, \dots, b_k\}$. We claim that $D=\{a_1, a_2, \dots, a_k\}$ is a dominating set of $G(V, E)$. If not, then there be a vertex $a_i\in V\backslash D$ such that the distance of $a_i$ to the nearest vertex $a_j$ in $D$ is greater than one. Therefore the vertex representing of $a_i$ and $a_j$ in $G^{'}(V^{'}, E^{'})$ must satisfies the the inequality $dist(b_i,b_j)>1$ where $b_j\in C$ and $b_i\notin C$. Hence $C$ is not a consistent subset because $dist(b_i, r_1)=1$, a contradiction.


% \end{proof}
% \begin{lemma}
%     The minimum consistent subset (\mcs) is $\log APX$ hard.
% \end{lemma}

% \begin{proof}
%     \cite{Fie} states that the dominating set is $\log APX$ hard for general graphs. Hence using lemma \ref{bubailemma6}, it is also proved that the minimum consistent subset (\mcs) is $\log APX$ hard.
% \end{proof}

==> treeold.tex <==
\section{\np-hardness of MCS for Trees}
In this section, we prove that \csp is \nph even when the input graph is a tree. We present a reduction from MAX-2SAT problem to \csp. Let $\theta$ be a given MAX-$2$SAT formula with $n$ variables $\{x_1, \ldots, x_n\}$ and $m$ clauses $\{c_1, \ldots, c_m\}$, $n,m \geq 50$ (\red{do we need this?}). We construct an instance $(T_{\theta}, C_{\theta})$ of the MCS problem from $\theta$ as follows.


%reduce an arbitrary given instance $\theta$ of the MAX-2SAT problem to an instance $(T_{\theta}, C_{\theta})$ of the MCS problem where $T_{\theta}$ is a tree. 

%Here,  $k$ clauses of $\theta$ can be satisfied if and only if the reduced tree $T$ has a consistent subset of a certain size (depending on $k$) that we describe later on.
%Throughout this section, by distance between two vertices in $T$, we refer to the hop-distance between them. The distance between a vertex $v$ and a path is the minimum distance between $v$ and any vertex of that path. The distance between two paths $P_1$ and $P_2$ in $T$ is the minimum distance of a pair vertices $v_1\in P_1$ and $v_2\in P_2$.


\begin{figure}[!htbp]
\centering
\includegraphics[width=0.8\textwidth]{treehardness.pdf}
\caption{An example of construction of $(T_{\theta}, C_{\theta})$ where $\theta=(x_1\lor x_2)\land (x_1\lor \overline{x_3})\land (\overline{x_2}\lor \overline{x_3}))$. For the assignment $x_1=x_2=x_3=\false$, we have shown the corresponding \cs with a red box around the vertices. For the mentioned assignment,  $(x_1\lor x_2)$ is not satisfied whereas the rest of the clauses are satisfied} \label{fig:red}
\end{figure}


%\subsection{Construction of $(T_{\theta}, C_{\theta})$}



\begin{tcolorbox}[breakable,bicolor,
  colback=cyan!5,colframe=cyan!5,title=Interval Graph Construction.,boxrule=0pt,frame hidden]


% \begin{mdframed}[backgroundcolor=cyan!5,topline=false,bottomline=false,leftline=false,rightline=false]
\noindent \underline{\textbf{\large Construction of $(T_{\theta}, C_{\theta})$.}}
%\noindent \paragraph{Reduction.}
%\subsection{Reduction}
\smallskip

\noindent The constructed tree $T_{\theta}$ is composed of variable and clause gadgets. 
\smallskip

\noindent {\bf Variable Gadget.}

\noindent A variable gadget $X_i$ for the variable $x_i \in \theta$ has two components, each component has a literal path, and $M$ pair of stabilizer vertices, as described below (see Figure \ref{fig:red}), where $M$ is very large.


\smallskip

\noindent {\bf Literal paths:}   A path (\red{define path}) $P_i^x=\langle x_i^1, x_i^2,x_i^3,x_i^4\rangle$ of four vertices, called the  \emph{positive literal path}, and a path $\overline{P}_i^x=\langle \overline{x}_i^1,\overline{x}_i^2,\overline{x}_i^3,\overline{x}_i^4\rangle$ of four vertices, called  the \emph{negative literal path}. All the vertices in $P_i^x$ are of color $c^x_i$ and all the vertices in $\overline{P}_i^x$ are of color $\overline{c}^x_i$.
 
 %In each path, all its nodes have the same color, and these two paths have different colors. The path $x_i$ corresponds to $x_i=1$, and path $\overline{x_i}$ corresponds to $\overline{x_i}=1$ (i.e. $x_i=0$).
\smallskip

\noindent {\bf Stabilizer vertices:} $M$ pairs of vertices $\{s_{i}^1, \overline{s}_i^1\}, \ldots, \{s_{i}^M, \overline{s}_i^M\}$ called the \emph{stabilizer vertices}. We will define the exact value of $M$ later. We set the color of each pair of vertices $\{s_{i}^j, \overline{s}_i^j\}$ to be $c^s(i,j)$. We denote the set of vertices $S_i=\{ s_{i}^1,  \ldots, s_{i}^M\}$ by  \emph{positive stabilizer vertices} and the set of vertices $\overline{S}_i=\{\overline{s}_i^1, \ldots,  \overline{s}_i^M\}$ by \emph{negative stabilizer vertices}. Each vertex in $S_i$ is connected to $x_i^1$ and each vertex in $\overline{S}_i$ is connected to $\overline{x}_i^1$.

The intuition behind this set of vertices is that by setting a large value of $M$ we ensure that either $s_{i}^1,  \ldots, \{s_{i}^M\}$ or $\{\overline{s}_i^1, \ldots,  \overline{s}_i^M\}$ is present in any "small" solution. 

%The vertices of the form $s_{i,j}^1$ are called the \emph{left stabilizers} while those of the form $s_{i,j}^2$ are called the right stabilizers. Each pair of stabilizer vertices have the same color, and these $M$ pairs of stabilizer vertices have distinct colour, which are also different from that of the vertices in variable paths and literal paths. The left (resp. right) stabilizer vertices are connected with the first vertex of left (resp. right) literal paths. 
%\end{description}

\smallskip

\noindent {\bf Clause Gadget.}

\noindent For each clause $C_i=(y_i\lor z_i)$ where $y_i$ and $z_i$ are two literals (positive/negative) present in $C_i$, we define the following gadget. It consists of three paths, namely \emph{left occurrence path} $P_i^Y=\langle y_i^1,\cdots y_i^7\rangle$, \emph{right occurrence path} $P_i^Z=\langle z_i^1,\cdots z_i^7\rangle$, and {\em clause path} $P_i^W=\langle w_i^1,\cdots w_i^7\rangle$ (see Figure \ref{fig:red}).
All the vertices in $P_i^Y$ and in $P_i^Z$ are of the same color as the corresponding literal path in their respective variable gadgets, that is for any literal $y_i$ (or $z_i$) in $C_i$ if $y_i=x_i$ ($z_i=x_i$) then we set the color of the vertices of $P_i^Y$ ($P_i^Z$) by $c_i^x$. If $y_i=\overline{x_i}$ ($z_i=\overline{x_i}$) then we set the color of the vertices of $P_i^Y$ ($P_i^Z$) by $\overline{c}_i^x$. We color the vertices in $P_i^W$ by $c^w_i$.
We connect $y_i^1$ with $w_i^2$ and $z_i^1$ to $w_i^6$ by an edge (see Figure \ref{fig:red}).









\smallskip

\noindent {\bf Central Vertex Gadget.}

\noindent We also have a central path $P^v=\langle v_1\cdots v_3\rangle$. For each variable $x_i$, $v_1$ is connected to $x_i^1$ and $\overline{x}_i^1$ (see Figure \ref{fig:red}). For each clause $C_i$, $v_1$ is connected to $w_i^4$. Color of the vertices of $P^v$  is $c^v$.


%\end{mdframed}

\end{tcolorbox}

% Another part of this reduction is a 
% vertex $v$, named central vertex, and it is attached with a path of length (including $v$), called the central path. The vertices of central path is different from all the  vertices in variable gadgets and clause gadgets. Now, we explain how the variable and clause gadgets are connected to form the tree $T$.

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.9\textwidth]{mcspic5a.pdf}
% \caption{A part of the reduction tree demonstrating one variable gadget $x_i$, and one clause gadget $c_\alpha$. For a truth assignment of $x_i=1$, the vertices included in the minimum consistent subset $S$ are enclosed with a square box. } \label{fig:red}
% \end{figure}

% \begin{enumerate}
% \item The two components of each variable gadget are individually connected with the central vertex $v$. 
% \item As mentioned earlier, the middle vertex of each clause gadget is connected with the central vertex $v$. 
% \end{enumerate}



Let us define $N(k)=n(M+2)+2k+3(n-k)+1$. Let $V_C$ be any consistent subset for $(T_{\theta}, C_{\theta})$ of size $N(k)$. Next, we prove a set of auxiliary claims about $V_C$. 


\begin{lemma}
        For any variable $x_i$, exactly one of the following is true.
        \begin{itemize}
            \item $S_i\subset V_C$, $\overline{S}_i\cap V_C=\emptyset$, and $x_i^2,\overline{x}_i^4\in V_C$. 
            \item $\overline{S}_i\subset V_C$, ${S}_i\cap V_C=\emptyset$, and $\overline{x}_i^2,x_i^4\in V_C$.
        \end{itemize}\label{lemma:exactlyone}
        
    \end{lemma}
    \begin{proof}
        
    \end{proof}

    \begin{lemma}
        $v_3\in V_C$.\label{lemma:v3invc}
    \end{lemma}
    \begin{proof}
        
    \end{proof}
    For any clause $C_i$, denote the corresponding clause gadget by $T_i^C=G[\{w_i^a,y_i^a,z_i^a|1\leq a\leq 7\}]$.
    \begin{lemma}
        For any clause $C_i$, $2\leq |V(T_i^C)\cap V_C|\leq 3$.\label{lemma:clause2or3}
    \end{lemma}
    \begin{proof}
    \end{proof}
Next, we prove the following theorem.

\begin{theorem}
    There exists an assignment to $\theta$ which satisfies at least $k$ clauses iff there is a consistent subset of size at most $N(k)$ for $(T_{\theta},C_{\theta})$.
\end{theorem}

\begin{proof}
    $ (\Rightarrow)$ For the forward direction, let there exist an assignment $A$ to $\theta$ that satisfies $k$ clauses. Consider the following set of vertices $V_A$. For each variable $x_i$ if $x_i$ is $\true$, include all the vertices in $S_i$ to $V_A$. Also include $x_i^2$ and $\overline{x}_i^4$ to $V_A$. If $x_i=\false$ then include all the vertices in $\overline{S}_i$ to $V_A$. Also include $x_i^4$ and $\overline{x}_i^2$ to $V_A$.

    For every satisfied clause $C_i=(y_i\lor z_i)$ wrt $A$ we include the following vertices to $V_A$. Without loss of generality assume that $y_i=\true$. We include $w_i^7$ and $z_i^1$ to $V_A$.
    For every unsatisfied clause $C_i=(y_i\lor z_i)$, we include the following vertices to $V_A$. We include $w_i^1$ $y_i^1$ and  $z_i^7$ to $V_A$. We also include $v_3$ into $V_A$.

    Observe that the cardinality of $V_A$ is $N(k)=n(M+2)+2k+3(n-k)+1$. Next, we prove that $V_A$ is a consistent subset for $T_{\theta}$. Observe that for any pair of vertices $(s_i^j,overline{s}_i^j)$, exactly one of them is in $V_A$. Without loss of generality assume that $s_i^j\in V_A$. Observe that $d(s_i^j,overline{s}_i^j)=d(overline{s}_i^j,V_A)=4$. If $x_i=\true$ then $d(x_i^j,x_i^2)\leq d(x_i^j,V_A)$ and $d(\overline{x}_i^j,\overline{x}_i^4)\leq d(\overline{x}_i^j,V_A)$. The case when $x_i=\false$ is symmetric.

    For any clause gadget either $w_i^1$ or $w_i^7$ is in $V_A$. Without loss of generality assume that $w_i^1\in V_A$. Observe that for every vertex $w_i^j$, $d(w_i^j,w_i^1)=d(w_i^j.V_A)$. Let $C_i=(y_i\lor z_i)$ be a satisfied clause and without loss of generality assume that $y_i=x_j=\true$. Observe that $d(y_i^3,x_j^2)=6$ and $d(y_i^3,V_A)=6$ and $d(y_i^a,x_j^2)=d(y_i^a,V_A)$.
    For any unsatisfied clause $C_i=(y_i\lor z_i)$ observe that $d(y_i^a,x_j^2)=d(y_i^a,V_A)$. Also for any $v_j$ where $1\leq j\leq 3$ $d(v_j,v_3)=d(v_j,V_A)$. Therefore $V_A$ is a consistent subset for $T_{\theta}$. 
    
    \smallskip
    \noindent $ (\Leftarrow) $ For the backward direction, let there beis a consistent subset $V_C$ of size at most $N(k)$ for $(T_{\theta},C_{\theta})$. 

    We known from Lemma~\ref{lemma:exactlyone} that either $S_i\subset V_C$ or $\overline{S}_i\subset V_C$.
    Consider the following assignment $A$ correspond to $V_C$. For any variable $x_i$ if $S_i\subset V_C$ we set $x_i=\true$, otherwise we set $x_i=\false$. 
    
    Observe that any clause $C_i$, $V_C$ either contains $w_i^1$ or $w_i^7$. Note that $|V_C|=n(M+2)+2k+3(n-k)+1$ and $V_C$ contains $M$ vertices from each variable gadget and $v_3\in V_C$ (follows from Lemma~\ref{lemma:v3invc} and Lemma~\ref{lemma:clause2or3}). From pigeonhole principle there exist $k$ clause $C_j=(y_j\lor z_j)$ such that either $V(P_j^Y)\cap V_C=\emptyset$ or  $V(P_j^Z)\cap V_C=\emptyset$. Without loss of generality assume that $C_1\cdots C_k$ be such clauses and for all $1\leq j\leq k$, $V(P_j^Y)\cap V_C=\emptyset$. Consider any clause $C_j$ where $1\leq j\leq k$. Without loss of generality assume $y_j=x_i$. Observe that $d(y_j^1,w_j^7)=6$. Thus $x_i^2\in V_C$ and hence $S_i\in V_C$. Therefore $x_i=\true$ in $A$. Hence $C_j$ is satisfied for the assignment $A$. Thus the claim holds.
\end{proof}



% \smallskip
% \noindent {\bf Intuition Behind the Construction.}

% \noindent We now give an intuition of this reduction. Observe that, each pair of stabilizer vertices has distinct color. If one of them in any side is selected in a consistent set $S$, then all of them in that side is to be selected irrespective of selection of other vertices in $T$ in $S$. Thus, in order to reduce the size of the consistent set, one needs to selected stabilizer vertices of one side only. Now, let us consider that the left stabilizer vertices are selected in the gadget $X_i$. in order to make the other stabilizer vertices and the vertices in the literal paths consistent, we need to do the following: 
% \begin{enumerate}
%  \item Select either first or second vertex ($x_{i,1}$ or $x_{i,2}$) of left literal path, fourth vertex of right literal path, and third vertex on the central path to make the variable gadget consistent. 
%  \item We will show below that by an appropriate choice of vertices in the clause gadget containing $x_i$, one can reduce the choice of vertex in the clause gadgets where  $x_i$ appears in uncomplemented form and $x_i=1$ is assigned in the formula $\theta$.  
% \end{enumerate}
% Similarly, if right stabilizer vertices are selected, we need to select the corresponding vertices in left and right literal paths, and it is possible to reduce selection of vertices in clause gadgets where $x_i$ appears in complemented form and $x_i=0$ is assigned in the formula $\theta$.  

% Here one more thing we mention that we select the third vertex of the central path. 

% Previous discussions say the following results for a satified MAX-2SAT formula $\theta$: 



% \begin{lemma} \label{lem:var}
% Each variable gadget, say $X_i$, contributes $M+2$ vertices in a minimum consistent set of $T$. 
% \end{lemma}
% \begin{proof}
% Follows from the fact that, depending on whether $x_i=1$ or $x_i=0$ is assigned in $\theta$, the MCS either contains the stabilizer vertices of the left component or right component, and accordingly the one vertex of each literal path is chosen.  
% \end{proof}

 

% \begin{lemma}\label{lem:clause}
% In the minimum consistent subset, the contribution of a satisfied clause $c_\alpha=l_i+l_j$ is exactly 2, and for a non-satisfied clause it is exactly 3. 
% \end{lemma}
% \begin{proof}
% {\bf First part:} A satisfied clause $c_\alpha=l_i+l_j$ has either one or two literals satisfied. 
% \begin{itemize}
%  \item If only one literal, say $l_i$ (uncomplemented or complemented $x_i$), is satisfied, then we include the first vertex $o_{\alpha,1}^j$ of the occurance path of $l_j$ and the end-vertex of the clause path in the side where occurance path of $l_j$ is connected, in the set $S$. Needless to say,  all the vertices of the occurance path of $l_j$ are satisfied. The first vertex of the occurance path of $l_i$ is satisfied due to the fact that (i) it is at a distance 6 or 7 from a vertex of same color in the variable gadget $X_i$, and (ii) is at a distance 8 from the selected vertex on the clause path. Thus, all the vertices of that occurance path are satisfied. The middle vertex of clause path is at distance 4 from the selected vertex of the clause path which is at least at the same distance from the selected vertex of any other color. Thus, here the contribution of $C_\alpha$ in $S$ is 2.
%  \item If both the literals $l_i$ and $l_j$ are satisfied, then we need to choose one vertex on the clause path to make the vertices on the clause path consistent. This forces to choose  a vertex on the occurance at atleast one side. We do the choice same as was done in the previous case. to make all the vertices in the clause path consistent. 
% \end{itemize}
% Thus, if $c_\alpha$ is satisfied all the vertices in the clause gadget $C_\alpha$ are consistently covered with 2 vertices in the minimum consistent set, and the first part follows.

% {\bf Second part:} If $c_\alpha$ is unsatisfied, the both the literals have value 0 in the truth assignment of variables in $\theta$. Thus, in the variable gadget $C_i$ and $C_j$, the vertex of color same as that of the path corresponding to $l_i$ and $l_j$ are at distance 8 from the first vertex ($o_{\alpha,1}^i$ and $o_{\alpha,1}^j$). Also, we have to make the vertices on the clause path consistent by choosing at least one vertex in that path. We choose any vertex (excepting three middle vertices $c_{\alpha,4},c_{\alpha,5},c_{\alpha,6}$) on the clause path, and accordingly one vertex in each of the occurance path is chosen. The reason of not choosing the three middle vertex in the clause path is that it makes the vertices on the central path inconsistent.  
% Thus, the second part of the lemma follows.
% \end{proof}

% Finally, the vertices in the central path also become consistent due to the choice of the vertex in that path as mentioned above.





% \begin{theorem} \label{lem:if}
% $T$ has a consistent subset of size at most $nM + 2n  + +1+3m - k$ if and only if at least $k$ clauses of $\theta$ can be satisfied.
% \end{theorem}

% \begin{proof}
% If part follows from Lemma \ref{lem:var} and \ref{lem:clause}, and an additional 1 in the count, that comes from the choice of a vertex on the central path in the minimum consistent set to make the vertices in that path consistent. The only if part follows from the choice of vertices in the set $S$ as described earlier, which makes all non-chosen vertices consistent.   
% \end{proof}

